EVINCE: Optimizing Multi-LLM Dialogues Using Conditional Statistics and Information Theory

EVINCE (Entropy and Variation IN Conditional Exchanges) is a novel framework for optimizing multi-LLM dialogues using conditional statistics and information theory. It addresses limitations in multi-agent debate (MAS) frameworks, where multiple LLMs chat without behavior modulation or mutual information quality assessment. Using dual entropy optimization to balance perspective diversity and prior knowledge, EVINCE provides quantitative tools to dynamically regulate LLM linguistic behaviors. When mutual information is low and both cross-entropy and Wasserstein distance are high, EVINCE promotes contentious dialogues to expose diverse perspectives and uncover inconsistencies. Conversely, as cross-entropy decreases and mutual information stabilizes, it transitions discussions into a conciliatory phase, encouraging compromise and acknowledgment of valid points. Using information-theoretic metrics and optimizing mutual information, EVINCE emerges as a structured and highly effective framework for multi-LLM collaboration.

==> Table-Contentiousness.tex <==

\begin{table*}[t!]
\vspace{-.1in}
\centering
\begin{footnotesize}
\begin{tabular}{|p{0.6cm}|p{3.6cm}|p{4.0cm}|p{4.0cm}|}
\toprule
\textbf{C.L.} & \textbf{Tone} & \textbf{Emphasis} & \textbf{Language} \\
\hline \hline
$0.9$ & Highly confrontational; focused on raising strong ethical, scientific, and social objections. & Flagging risks and downsides; ethical quandaries, unintended consequences, and exacerbation of inequalities. & Definitive and polarizing, e.g., ``should NOT be allowed,'' ``unacceptable risks,'' ``inevitable disparities.'' \\
\hline
$0.7$ & Still confrontational but more open to potential benefits, albeit overshadowed by negatives. & Acknowledging that some frameworks could make it safer or more equitable, while cautioning against its use. & Less polarizing; ``serious concerns remain,'' ``needs more scrutiny.'' \\
\hline
0.5 & Balanced; neither advocating strongly for nor against gene editing. & Equal weight on pros and cons; looking for a middle ground. & Neutral; ``should be carefully considered,'' ``both benefits and risks.'' \\
\hline
0.3 & More agreeable than confrontational, but maintaining reservations. & Supportive but cautious; focus on ensuring ethical and equitable use. & Positive but careful; ``transformative potential,'' ``impetus to ensure.'' \\
\hline
0.0 & Completely agreeable and supportive. & Fully focused on immense potential benefits; advocating for proactive adoption. & Very positive; ``groundbreaking advance,'' ``new era of possibilities.'' \\
\bottomrule
\end{tabular}
\end{footnotesize}
\vspace{-.05in}
\caption{Changes in linguistic behaviors of LLMs at different contentiousness levels.}
\label{tab:contentiousness}
\vspace{-.15in}
\end{table*}    

%\section*{Appendix G: Contentiousness Parameter Modulation}

\begin{comment}

Table~\ref{tab:contentiousness} presents 
how an LLM adjusts its linguistic behavior 
after the value of the ``contentiousness'' parameter.
By modulating contentiousness, it has been shown
that an LLM can condition itself to 
adapt to different linguistic behaviors to
achieve a new establish goal and context.
Details are presented in \cite{SocraSynthChang2023} and
also illustrated in Section~\ref{sec:exp}.
    
\end{comment}
